Never Trust Your Victim: Weaponizing Vulnerabilities in Security Scanners

The first step of every attack is reconnaissance, i.e., to acquire information about the target. A common belief is that there is almost no risk in scanning a target from a remote location. In this paper we falsify this belief by showing that scanners are exposed to the same risks as their targets. Our methodology is based on a novel attacker model where the scan author becomes the victim of a counter-strike. We developed a working prototype, called RevOK, and we applied it to 78 scanning systems. Out of them, 36 were found vulnerable to XSS. Remarkably, RevOK also found a severe vulnerability in Metasploit Pro, a mainstream penetration testing tool.

==> data/corr-matix-nonumbers.tex <==
% GNUPLOT: LaTeX picture
\setlength{\unitlength}{0.240900pt}
\ifx\plotpoint\undefined\newsavebox{\plotpoint}\fi
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\begin{picture}(1500,900)(0,0)
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\put(550,552){\usebox{\plotpoint}}
\put(1288,552){\usebox{\plotpoint}}
\put(530,552){\makebox(0,0)[r]{Status Message}}
\put(550,575){\usebox{\plotpoint}}
\put(1288,575){\usebox{\plotpoint}}
\put(530,575){\makebox(0,0)[r]{Server}}
\put(550,598){\usebox{\plotpoint}}
\put(1288,598){\usebox{\plotpoint}}
\put(530,598){\makebox(0,0)[r]{X-Powered-By}}
\put(550,621){\usebox{\plotpoint}}
\put(1288,621){\usebox{\plotpoint}}
\put(530,621){\makebox(0,0)[r]{Location}}
\put(550,643){\usebox{\plotpoint}}
\put(1288,643){\usebox{\plotpoint}}
\put(530,643){\makebox(0,0)[r]{Set-Cookie}}
\put(550,666){\usebox{\plotpoint}}
\put(1288,666){\usebox{\plotpoint}}
\put(530,666){\makebox(0,0)[r]{X-Content-Type-Options}}
\put(550,689){\usebox{\plotpoint}}
\put(1288,689){\usebox{\plotpoint}}
\put(530,689){\makebox(0,0)[r]{X-AspNet-Version}}
\put(550,711){\usebox{\plotpoint}}
\put(1288,711){\usebox{\plotpoint}}
\put(530,711){\makebox(0,0)[r]{X-AspNetMvc-Version}}
\put(550,734){\usebox{\plotpoint}}
\put(1288,734){\usebox{\plotpoint}}
\put(530,734){\makebox(0,0)[r]{X-Varnish}}
\put(550,757){\usebox{\plotpoint}}
\put(1288,757){\usebox{\plotpoint}}
\put(530,757){\makebox(0,0)[r]{Strict-Transport-Security}}
\put(550,780){\usebox{\plotpoint}}
\put(1288,780){\usebox{\plotpoint}}
\put(530,780){\makebox(0,0)[r]{Content-Security-Policy}}
\put(550,802){\usebox{\plotpoint}}
\put(1288,802){\usebox{\plotpoint}}
\put(530,802){\makebox(0,0)[r]{X-XSS-Protection}}
\put(550,825){\usebox{\plotpoint}}
\put(1288,825){\usebox{\plotpoint}}
\put(530,825){\makebox(0,0)[r]{X-Frame-Options}}
\put(550,848){\usebox{\plotpoint}}
\put(1288,848){\usebox{\plotpoint}}
\put(530,848){\makebox(0,0)[r]{Body}}
\put(576,541){\usebox{\plotpoint}}
\put(576,859){\usebox{\plotpoint}}
\put(576,521){\makebox(0,0)[r]{Status Message}}
\put(629,541){\usebox{\plotpoint}}
\put(629,859){\usebox{\plotpoint}}
\put(629,521){\makebox(0,0)[r]{Server}}
\put(682,541){\usebox{\plotpoint}}
\put(682,859){\usebox{\plotpoint}}
\put(682,521){\makebox(0,0)[r]{X-Powered-By}}
\put(735,541){\usebox{\plotpoint}}
\put(735,859){\usebox{\plotpoint}}
\put(735,521){\makebox(0,0)[r]{Location}}
\put(787,541){\usebox{\plotpoint}}
\put(787,859){\usebox{\plotpoint}}
\put(787,521){\makebox(0,0)[r]{Set-Cookie}}
\put(840,541){\usebox{\plotpoint}}
\put(840,859){\usebox{\plotpoint}}
\put(840,521){\makebox(0,0)[r]{X-Content-Type-Options}}
\put(893,541){\usebox{\plotpoint}}
\put(893,859){\usebox{\plotpoint}}
\put(893,521){\makebox(0,0)[r]{X-AspNet-Version}}
\put(945,541){\usebox{\plotpoint}}
\put(945,859){\usebox{\plotpoint}}
\put(945,521){\makebox(0,0)[r]{X-AspNetMvc-Version}}
\put(998,541){\usebox{\plotpoint}}
\put(998,859){\usebox{\plotpoint}}
\put(998,521){\makebox(0,0)[r]{X-Varnish}}
\put(1051,541){\usebox{\plotpoint}}
\put(1051,859){\usebox{\plotpoint}}
\put(1051,521){\makebox(0,0)[r]{Strict-Transport-Security}}
\put(1104,541){\usebox{\plotpoint}}
\put(1104,859){\usebox{\plotpoint}}
\put(1104,521){\makebox(0,0)[r]{Content-Security-Policy}}
\put(1156,541){\usebox{\plotpoint}}
\put(1156,859){\usebox{\plotpoint}}
\put(1156,521){\makebox(0,0)[r]{X-XSS-Protection}}
\put(1209,541){\usebox{\plotpoint}}
\put(1209,859){\usebox{\plotpoint}}
\put(1209,521){\makebox(0,0)[r]{X-Frame-Options}}
\put(1262,541){\usebox{\plotpoint}}
\put(1262,859){\usebox{\plotpoint}}
\put(1262,521){\makebox(0,0)[r]{Body}}
\put(550.0,541.0){\rule[-0.200pt]{0.400pt}{76.606pt}}
\put(550.0,541.0){\rule[-0.200pt]{177.784pt}{0.400pt}}
\put(1288.0,541.0){\rule[-0.200pt]{0.400pt}{76.606pt}}
\put(550.0,859.0){\rule[-0.200pt]{177.784pt}{0.400pt}}
\put(550.0,541.0){\rule[-0.200pt]{0.400pt}{76.606pt}}
\put(550.0,541.0){\rule[-0.200pt]{177.784pt}{0.400pt}}
\put(1288.0,541.0){\rule[-0.200pt]{0.400pt}{76.606pt}}
\put(550.0,859.0){\rule[-0.200pt]{177.784pt}{0.400pt}}
\end{picture}


==> experiments.tex <==
\section{Experimental assessment + Case study (Metasploit)}\label{sec:experiments}

\subsection{From vuln to exploit}


==> figs/tainted-vulnerable.tex <==
% This file was created by tikzplotlib v0.9.1.
\begin{tikzpicture}


\definecolor{color0}{rgb}{0.7, 0.7, 0.7}
\definecolor{color1}{rgb}{1,1,1}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-0.98, xmax=13.98,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9,10,11,12,13},
xticklabel style = {rotate=90.0},
height=0.5\columnwidth,
width=\columnwidth,
xticklabels={
	Status Message,
	Server,
	X-Powered-By,
	Location,
	Set-Cookie,
	X-Content-Type,
	X-AspNet-Version,
	X-AspNetMvc-Version,
	X-Varnish,
	Strict-Transport-Security,
	Content-Security-Policy,
	X-XSS-Protection,
	X-Frame-Options,
	Body
},
y grid style={white!69.0196078431373!black},
ymin=0, ymax=61.95,
ytick style={color=black}
]
\draw[draw=black,fill=color0] (axis cs:-0.3,0) rectangle (axis cs:0.3,21);
\draw[draw=black,fill=color0] (axis cs:0.7,0) rectangle (axis cs:1.3,26);
\draw[draw=black,fill=color0] (axis cs:1.7,0) rectangle (axis cs:2.3,21);
\draw[draw=black,fill=color0] (axis cs:2.7,0) rectangle (axis cs:3.3,21);
\draw[draw=black,fill=color0] (axis cs:3.7,0) rectangle (axis cs:4.3,17);
\draw[draw=black,fill=color0] (axis cs:4.7,0) rectangle (axis cs:5.3,10);
\draw[draw=black,fill=color0] (axis cs:5.7,0) rectangle (axis cs:6.3,20);
\draw[draw=black,fill=color0] (axis cs:6.7,0) rectangle (axis cs:7.3,19);
\draw[draw=black,fill=color0] (axis cs:7.7,0) rectangle (axis cs:8.3,19);
\draw[draw=black,fill=color0] (axis cs:8.7,0) rectangle (axis cs:9.3,19);
\draw[draw=black,fill=color0] (axis cs:9.7,0) rectangle (axis cs:10.3,19);
\draw[draw=black,fill=color0] (axis cs:10.7,0) rectangle (axis cs:11.3,19);
\draw[draw=black,fill=color0] (axis cs:11.7,0) rectangle (axis cs:12.3,16);
\draw[draw=black,fill=color0] (axis cs:12.7,0) rectangle (axis cs:13.3,1);
\draw[draw=black,fill=color1] (axis cs:-0.3,21) rectangle (axis cs:0.3,41);
\draw[draw=black,fill=color1] (axis cs:0.7,26) rectangle (axis cs:1.3,51);
\draw[draw=black,fill=color1] (axis cs:1.7,21) rectangle (axis cs:2.3,49);
\draw[draw=black,fill=color1] (axis cs:2.7,21) rectangle (axis cs:3.3,59);
\draw[draw=black,fill=color1] (axis cs:3.7,17) rectangle (axis cs:4.3,39);
\draw[draw=black,fill=color1] (axis cs:4.7,10) rectangle (axis cs:5.3,25);
\draw[draw=black,fill=color1] (axis cs:5.7,20) rectangle (axis cs:6.3,46);
\draw[draw=black,fill=color1] (axis cs:6.7,19) rectangle (axis cs:7.3,44);
\draw[draw=black,fill=color1] (axis cs:7.7,19) rectangle (axis cs:8.3,43);
\draw[draw=black,fill=color1] (axis cs:8.7,19) rectangle (axis cs:9.3,42);
\draw[draw=black,fill=color1] (axis cs:9.7,19) rectangle (axis cs:10.3,44);
\draw[draw=black,fill=color1] (axis cs:10.7,19) rectangle (axis cs:11.3,42);
\draw[draw=black,fill=color1] (axis cs:11.7,16) rectangle (axis cs:12.3,38);
\draw[draw=black,fill=color1] (axis cs:12.7,1) rectangle (axis cs:13.3,14);
\end{axis}

\end{tikzpicture}

